On the Wick Rotation of the Four-point Function in Conformal Field Theories

Conformal field theories (CFTs) in Euclidean signature satisfy well-accepted rules, such as conformal invariance and the convergent Euclidean operator product expansion (OPE). Nowadays, it is common to assume that CFT correlators exist and have various properties in the Lorentzian signature. Some of these properties may represent extra assumptions, and it is an open question if they hold for familiar statistical-physics CFTs such as the critical 3d Ising model. In this thesis, we clarify that at the level of four-point functions, the Euclidean CFT axioms imply the standard quantum field theory axioms such as Osterwalder-Schrader axioms (in Euclidean) and Wightman axioms (in Lorentzian).

==> notation.tex <==
\nnchapter{Notations and conventions}
\thispagestyle{fancy}
\section*{Coordinates}
We will mostly work in Euclidean signature. Under this convention, Euclidean points are real vectors
\begin{equation*}
	\begin{split}
		x=(\tau,\mathbf{x})\in\mathbb{R}^d
	\end{split}
\end{equation*}
Here $\tau\in\mathbb{R}$ is the Euclidean time and $\mathbf{x}\in\mathbb{R}^{d-1}$ is the spatial part. $x^2$ is the sum of squares of all components
\begin{equation*}
	\begin{split}
		x^2=\tau^2+\mathbf{x}^2.
	\end{split}
\end{equation*}
For Lorentzian points, the time variables are imaginary: $x=(i t,\mathbf{x})$. Thus we use $(-+\cdots+)$ signature for the Lorentzian metric
\begin{equation*}
	\begin{split}
		x^2=-t^2+\mathbf{x}^2.
	\end{split}
\end{equation*}
We use the letter ``c" to denote the n-point configurations: $c=(x_1,x_2,\ldots,x_n)$. We let $c_E$ denote Euclidean configurations and $c_L$ denote Lorentzian configurations.

For a four-point configuration $c=(x_1,x_2,x_3,x_4)$, we use the standard notation for cross-ratio variables: $(u,v), (z,\bar{z}), (\rho,\bar{\rho})$, defined by
\begin{equation*}
	\begin{split}
		u=&\dfrac{x_{12}^2\,x_{34}^2}{x_{13}^2\,x_{24}^2},\quad v=\dfrac{x_{14}^2\,x_{23}^2}{x_{13}^2\,x_{24}^2},\\
		u=&z\bar{z},\quad v=(1-z)(1-\bar{z}),\\
		\rho=&\dfrac{z}{(1+\sqrt{1-z})^2},\quad\bar{\rho}=\dfrac{\bar{z}}{(1+\sqrt{1-\bar{z}})^2}.
	\end{split}
\end{equation*} 

\section*{Sets}
We will consider several sets of configurations. The forward tube is
\begin{equation*}
	\begin{split}
		\mathcal{T}_n=\left\{c=(x_1,\ldots,x_n)\in\mathbb{C}^{nd}\Big{|}\mathrm{Re}(x_k^0-x_{k+1}^0)>\abs{\mathrm{Im}(\mathbf{x}_k-\mathbf{x}_{k+1})},\,k=1,2,\ldots,n\right\}.
	\end{split}
\end{equation*}
We will also consider the subset of $\mathcal{T}_n$ where the spatial components are real
\begin{equation*}
	\begin{split}
		\mathcal{D}_n=\left\{c\in\mathcal{T}_n\Big{|}\mathrm{Im}(\mathbf{x}_k)=0,\,k=1,2,\ldots,n\right\}.
	\end{split}
\end{equation*}
In the thesis, we will mainly consider the four-point function. If we do not specify the lower indices, by ``$\mathcal{D}$" we mean ``$\mathcal{D}_4$".

The set of Euclidean 4-point configurations with time-ordering is
\begin{equation*}
	\begin{split}
		\mathcal{D}_E=\left\{c_E=(x_1,x_2,x_3,x_4)\in\mathbb{R}^{4d}\Big{|}x_1^0>x_2^0>x_3^0>x_4^0\right\}.
	\end{split}
\end{equation*}
The set of Lorentzian four-point configurations is
\begin{equation*}
	\begin{split}
		\mathcal{D}_L=\left\{c_L=(x_1,x_2,x_3,x_4)\Big{|}x_k=(it_k,\mathbf{x}_k)\in i\mathbb{R}\times\mathbb{R}^{d-1},\,k=1,2,3,4\right\}.
	\end{split}
\end{equation*}
In the analytic continuation problem described in the thesis, we will consider the following set of four-point configurations
\begin{equation*}
	\begin{split}
		\Gamma = \{ c \in \mathcal{T}_4 : [1 + u (c) - v (c)]^2 - 4 u (c) = 0 \},
	\end{split}
\end{equation*}
where $u$ and $v$ are the cross-ratios of the four-point configuration $c$.

\section*{Functions}
The Euclidean $n$-point function is denoted by $G_n^E(x_1,\ldots,x_n)$ or $G_n^E(c_E)$, where $c_E=(x_1,\ldots,x_n)\in\mathbb{R}^{nd}$ is a Euclidean $n$-point configuration.

We will use two kinds of $\theta$-functions. The first one is defined on the real axis:
\begin{equation*}
	\begin{split}
		\theta(x)=\begin{cases}
			1,\qquad x\geqslant0, \\ 0,\qquad x<0.
		\end{cases}
	\end{split}
\end{equation*} 
The second one is defined in the Lorentzian momentum space
\begin{equation*}
	\begin{split}
		\theta_{V_+}(p)=\begin{cases}
			p,\qquad p\in\overline{V}_+, \\ 0,\qquad p\notin\overline{V}_+.
		\end{cases}
	\end{split}
\end{equation*} 



